Perturbation theory for the $\Phi^4_3$ measure, revisited with Hopf algebras

We give a relatively short, almost self-contained proof of the fact that the partition function of the suitably renormalised $\Phi^4_3$ measure admits an asymptotic expansion, the coefficients of which converge as the ultraviolet cut-off is removed. We also examine the question of Borel summability of the asymptotic series. The proofs are based on Wiener chaos expansions, Hopf-algebraic methods, and bounds on the value of Feynman diagrams obtained through BPHZ renormalisation.

==> Borel.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we examine the question of whether the asymptotic 
expansion~\eqref{eq:cumulant}, though not convergent, can nevertheless be 
related to a convergent quantity. A positive answer to this question can be 
given thanks to the theory of Borel summation. This fact has been known in 
quantum field theory for quite a while, though first proofs of Borel summability 
for the $\Phi^4_2$ and $\Phi^4_3$ 
model~\cite{Eckmann_Magnen_Seneor_75,Magnen_Seneor_77} were quite difficult. 
Here we show that with modern analytical tools, which combine Hopf-algebraic 
methods, an improved Borel summation result by Sokal~\cite{Sokal80}, and a 
decomposition originally obtained by Hepp in~\cite{Hepp66}, the proof of Borel 
summability can be simplified considerably. The analytical arguments are 
strongly based on the presentation in~\cite{Hairer_BPHZ}, made more 
quantitative in~\cite{Berglund_Bruned_19}. 

We start in Section~\ref{ssec:zerodim} by presenting the main ideas of Borel 
summation, and the result by Sokal, in the case of the zero-dimensional $\Phi^4$ 
model, whose partition function is simply an integral over $\R$. See 
also~\cite{Rivasseau_09} for a more detailed account of various resummation 
techniques for that model. Then we show in Section~\ref{ssec:dimthree} how these 
methods can be extended to the three-dimensional case, using in particular 
methods introduced by Hepp. 


\subsection{The case of the $\Phi^4_0$ model} 
\label{ssec:zerodim} 

The $\Phi^4_0$ model is simply the $\Phi^4$ model for a field $\phi$ defined at 
a single point. Its potential is 
\begin{equation}
V(\phi) = \frac12\phi^2 + \frac{\eps}{4}\phi^4\;, 
\end{equation} 
and its partition function is given by 
\begin{equation}
Z(\eps) = \int_{-\infty}^\infty \e^{-V(\phi)} \6\phi
= \int_{-\infty}^\infty \e^{-\phi^2/2} \e^{-\eps\phi^4/4} \6\phi\;.
\end{equation} 
The integral is clearly well-defined for $\eps \geqs 0$. It can also be 
extended to complex values of $\eps$, at least if $\re\eps\geqs0$, and possibly 
to other complex values. However, the integral is clearly not convergent for 
real $\eps < 0$. Therefore, $Z$ is not analytic in a neighbourhood of $\eps = 
0$, and does not admit a convergent expansion in powers of $\eps$. 

If we nevertheless expand the exponential, we obtain 
\begin{equation}
Z(\eps) 
\asymp \sum_{n\geqs0} \frac{1}{n!} \biggpar{-\frac{\eps}{4}}^n 
\int_{-\infty}^\infty \phi^{4n} \e^{-\phi^2/2} \6\phi \;,
\end{equation}
where the symbol $\asymp$ denotes an asymptotic expansion. We can interpret 
$\e^{-\phi^2/2}$ as the density of a Gaussian measure (up to normalisation), 
which yields 
\begin{align}
Z(\eps) 
&\asymp \sqrt{2\pi}\sum_{n\geqs0} \frac{1}{n!} 
\biggpar{-\frac{\eps}{4}}^n 
\bigexpecin{\mu}{\phi^{4n}} \\
&= \sqrt{2\pi}\sum_{n\geqs0} \biggpar{-\frac{\eps}{4}}^n 
\frac{(4n-1)!!}{n!} \;,
\end{align}
where $(4n-1)!!$ is defined in~\eqref{eq:double_factorial}, and we have used 
the Isserlis--Wick theorem to compute the moments of the normal law. Recalling 
that $n! = \Gamma(n+1)$ and using~\eqref{eq:double_factorial}, 
% the relation 
% \begin{equation}
% (4n-1)!! = \frac{(4n)!}{2^{2n}(2n)!}
% = \frac{\Gamma(4n+1)}{2^{2n} \Gamma(2n+1)}
% \end{equation} 
% which follows from separating even and odd factors in $(4n)!$, 
we get 
\begin{equation}
Z(\eps) \asymp 
\sqrt{2\pi}\sum_{n\geqs0} \biggpar{-\frac{\eps}{16}}^n 
\frac{\Gamma(4n+1)}{\Gamma(2n+1)\Gamma(n+1)}\;.
\end{equation} 
The general term of this formal series can be analysed by using Legendre's 
duplication formula for the Gamma function 
\begin{equation}
\Gamma(2z) = \frac{1}{\sqrt{\pi}} 2^{2z-1} 
\Gamma(z)\Gamma(z+\tfrac12)\;,
\end{equation} 
which yields 
\begin{equation}
\Gamma(4n+1) = 4n \Gamma(4n) 
= \frac{2}{\sqrt{\pi}} n 2^{4n} \Gamma(2n)\Gamma(2n+\tfrac12)\;.
\end{equation} 
Therefore 
\begin{align}
Z(\eps) 
&\asymp 2 \sqrt{2} \sum_{n\geqs0} (-\eps)^n 
\frac{n\Gamma(2n)\Gamma(2n+\tfrac12)}{\Gamma(n+1)\Gamma(2n+1)} \\
\label{eq:Zeps}
&= \sqrt{2} \sum_{n\geqs0} (-\eps)^n 
\frac{\Gamma(2n+\tfrac12)}{\Gamma(n+1)} \\
&= \frac1{\sqrt{\pi}} \sum_{n\geqs0} (-4\eps)^n 
\frac{\Gamma(n+\tfrac14)\Gamma(n+\tfrac34)}{\Gamma(n+1)}\;,
\end{align}
where we used $2n\Gamma(2n) = \Gamma(2n+1)$ to get the second line. 
Stirling's formula implies 
\begin{equation}
\Gamma(z+\alpha) = z^\alpha \Gamma(z) \biggbrak{1 + 
\biggOrder{\frac{\alpha-1}{z}}}\;,
\end{equation} 
showing that the general term in the series~\eqref{eq:Zeps} diverges like 
$\Gamma(n)$. Therefore, the series is indeed divergent. 

\begin{remark}
A more direct way of obtaining the asymptotic expansion~\eqref{eq:Zeps} is to 
notice that 
\begin{equation}
\label{eq:Z_Laplace} 
Z(\eps) 
= 2 \int_0^\infty \e^{-\phi^2/2} \e^{-\eps\phi^4/4} \6\phi
= \sqrt{2}\int_0^\infty \e^{-t} \frac{\e^{-\eps t^2}}{\sqrt{t}} 
\6t\;,
\end{equation} 
where we have used the change of variables $\phi = \sqrt{2t}$. Expanding 
the exponential, we obtain 
\begin{equation}
Z(\eps) 
\asymp \sqrt{2}\sum_{n\geqs0} \frac{(-\eps)^n}{n!}\int_0^\infty 
t^{2n-\frac12} 
\e^{-t}\6t
= \sqrt{2}\sum_{n\geqs0} (-\eps)^n \frac{\Gamma(2n+\frac12)}{n!}
\end{equation} 
which agrees with~\eqref{eq:Zeps}. 
\end{remark}

Certain divergent series can be resummed by a procedure known as Borel 
summation. Consider a formal power series 
\begin{equation}
A(\eps) = \sum_{n\geqs0} a_n \eps^n\;.
\end{equation} 
We can rewrite it as 
\begin{equation}
A(\eps) = \sum_{n\geqs0} a_n\eps^n \frac{\Gamma(n+1)}{n!}  
= \sum_{n\geqs0} \frac{a_n\eps^n}{n!} \int_0^\infty t^n \e^{-t} \6t\;.
\end{equation} 
Define the Borel-transformed power series by interchanging the sum and the 
integral, that is 
\begin{equation}
A_{\text{Borel}}(\eps) 
:= \int_0^\infty \e^{-t} \sum_{n\geqs0} \frac{a_n\eps^nt^n}{n!} \6t 
= \int_0^\infty \e^{-t} \cB A(\eps t) \6t\;, 
\end{equation} 
which is the Laplace transform of the Borel sum 
\begin{equation}
\cB A(t) := \sum_{n\geqs0} \frac{a_n}{n!}t^n\;.
\end{equation} 
Watson's theorem~\cite{Watson_1912} gives conditions under which 
$A_{\text{Borel}}(\eps)$ admits the asymptotic series $A(\eps)$. 

In the case of the expansion~\eqref{eq:Zeps} we find 
\begin{equation}
\label{eq:BZt} 
\cB Z(t) = \frac{1}{\sqrt{\pi}} \sum_{n\geqs0} b_n t^n\;,
\end{equation} 
where
\begin{equation}
b_n = (-4)^n \frac{\Gamma(n+\tfrac14)\Gamma(n+\tfrac34)}{\Gamma(n+1)^2}
= \frac{(-4)^n}{n} \biggpar{1 + \biggOrder{\frac1n}}\;.
\end{equation} 
The series~\eqref{eq:BZt} has radius of convergence $\frac14$, with a pole 
located at $-\frac14$. One can thus expect that it admits an analytic 
continuation to a domain including all positive reals, so that its Laplace 
transform indeed converges. 

In~\cite{Sokal80}, Alan Sokal has proved the following improvement of 
Watson's theorem. Assume that $A$ is analytic in a disc $D_R = 
\setsuch{\eps}{\re\eps^{-1} > R^{-1}}$, which is 
tangent to the imaginary axis. Assume further that $A$ admits the 
asymptotic expansion 
\begin{equation}
\label{eq:asympt_Sokal} 
A(\eps) = \sum_{k=0}^{n-1} a_k \eps^k + R_n(\eps)\;,
\end{equation} 
where
\begin{equation}
\label{eq:bound_Sokal} 
\bigabs{R_n(\eps)} 
\leqs C r^n n! \abs{\eps}^n
\end{equation} 
for some $C, r>0$, uniformly in $n$ and $\eps$ in $D_R$. Then $\cB A(t)$ 
converges for $\abs{t} < 1/r$, and has an analytic continuation to a 
$1/r$-neighbourhood of the positive real axis. Furthermore, $A$ can be 
represented by the absolutely convergent integral 
\begin{equation}
A(\eps) = \frac{1}{\eps} \int_0^\infty \e^{-t/\eps} \cB A(t) \6t
\end{equation} 
for any $\eps\in D_R$. 

To apply this to our situation, we write 
\begin{equation}
\frac{Z(\eps)}{\sqrt{2\pi}} 
= \sum_{k=0}^{n-1} \frac{1}{k!} 
\biggpar{-\frac{\eps}{4}}^n \bigexpec{\phi^{4k}} 
+ \Biggexpec{\e^{-\eps\phi^4/4} - \sum_{k=0}^{n-1} \frac{1}{k!} 
\biggpar{-\frac{\eps}{4}}^k \phi^{4k}}\;.
\end{equation} 
We then use the fact that for any $n\in\N$, one has the Taylor expansion  
\begin{align}
 \e^{-z} 
 &= \sum_{k=0}^{n-1} \frac{1}{k!}(-z)^k
 + (-z)^n \int_0^1 \int_0^{t_1} \dots \int_0^{t_{n-1}} 
 \e^{-t_n z} \6t_n\dots\6t_1 \\
 &= \sum_{k=0}^{n-1} \frac{1}{k!}(-z)^k
 + (-z)^n \int_0^1 \int_0^1 \dots \int_0^1 s_1 \dots s_{n-1}
 \e^{-s_1\dots s_n z} \6s_n\dots\6s_1\;,
 \label{eq:Taylor_remainder} 
\end{align} 
showing that for any $z$ with positive real part, 
\begin{equation}
\Biggabs{\e^{-z} - \sum_{k=0}^{n-1} \frac{1}{k!}(-z)^k} 
\leqs \frac{1}{n!} \abs{z}^n\;.
\end{equation} 
This implies that $Z(\eps)/\sqrt{2\pi}$ satisfies~\eqref{eq:asympt_Sokal} with 
a remainder $R_n$ such that  
\begin{equation}
\bigabs{R_n(\eps)} 
\leqs \frac{1}{n!} \Biggpar{\frac{\abs{\eps}}{4}}^n 
\bigexpec{\phi^{4n}}\;.
\end{equation} 
By the above computations, the remainder indeed meets Sokal's conditions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The case of the $\Phi^4_3$ model} 
\label{ssec:dimthree} 

As mentioned above, Borel summability of the perturbation expansions of 
correlation functions (or Schwinger functions) of the $\Phi^4_d$ model has been 
proved in~\cite{Eckmann_Magnen_Seneor_75} in the case $d=2$, and 
in~\cite{Magnen_Seneor_77} in the case $d=3$. The proofs are based on cluster 
expansion techniques from statistical physics, and are quite technical. Here we 
outline a comparatively simple proof of Borel summability of the expansion of 
the partition function, based on the techniques described above. The essential 
(and non-trivial) analytical ingredient is a bound on the value of 
BPHZ-renormalised Feynman diagrams, explained in~\cite{Hairer_BPHZ}, and made 
more quantitative in~\cite{Berglund_Bruned_19}. 

We start by observing that for any $n\geqs1$, we have the Taylor expansion 
\begin{equation}
 \e^{-\alpha X} = S_n^0 + R_n^0\;, 
 \qquad 
 S_n^0 = \sum_{p=0}^{n-1} \frac{(-\alpha)^p}{p!} X^p\;, \qquad 
 R_n^0 = \frac{(-\alpha)^n}{n!} X^n r_n(X)\;,
\end{equation} 
with a remainder satisfying $r_n(X) = \e^{-\theta(X)\alpha X}$ for some 
$\theta(X)\in[0,1]$. Disregarding for the moment any questions related to 
renormalisation, we note that 
\begin{equation}
 \log \expec{\e^{-\alpha X}} - \log \expec{S_n^0}
= \log\frac{\expec{\e^{-\alpha X}}}{\expec{S_n^0}} 
= \log \Biggpar{1 + \frac{\expec{R_n^0}}{\expec{S_n^0}}}\;.
\end{equation}
The Cauchy--Schwarz inequality yields 
\begin{equation}
 \bigabs{\expec{R_n^0}}
 \leqs \frac{\abs{\alpha}^n}{n!} 
 \sqrt{\expec{X^{2n}} \expec{r_n(X)^2}}\;, 
\end{equation} 
so that since $\log(1+\abs{x}) \leqs \abs{x}$, we obtain the bound 
\begin{equation}
 \Bigabs{\log \expec{\e^{-\alpha X}} - \log \expec{S_n^0}}
 \leqs \frac{\abs{\alpha}^n}{n!} \sqrt{\expec{X^{2n}}}
 \frac{\sqrt{\expec{r_n(X)^2}}}{\expec{S_n^0}}
\end{equation} 
on the remainder of the cumulant expansion. Note in particular 
that~\eqref{eq:Taylor_remainder} implies 
\begin{align}
 \frac{\expec{r_n(X)^2}}{\expec{S_n^0}^2}
 &= (n!)^2 \int_{[0,1]^{2n}} s_1\dots s_{n-1} \tilde s_1\dots \tilde s_{n-1}
 \frac{\expec{\e^{-[s_1\dots s_n + \tilde s_1\dots \tilde s_n]\alpha X}}}
 {\expec{S_n^0}^2} \6s\6\tilde s \\
 &\leqs \sup_{(s,\tilde s) \in [0,1]^{2n}} 
 \frac{\expec{\e^{-[s_1\dots s_n + \tilde s_1\dots \tilde s_n]\alpha X}}}
 {\expec{S_n^0}^2}\;,
 \label{eq:CS_remainder} 
\end{align} 
which one would expect to have order $1$ if no renormalisation were needed.

We now want to transpose this idea to the situation with renormalisation. 
Applying the linear map $\cM\circ\chi_\eta$ to $\e^{-\alpha X}$, we obtain 
\begin{equation}
 \e^{-\alpha X - \beta Y} 
 = (\cM \circ \chi_\eta) (S_n^0) + (\cM \circ \chi_\eta) (R_n^0)
 =: S_n + R_n\;.
\end{equation} 
By the same computation as above, we have 
\begin{equation}
 \log \expec{\e^{-\alpha X - \beta Y}} 
 = \log \expec{S_n} + \log\Biggpar{1 + \frac{\expec{R_n}}{\expec{S_n}}}\;,
\end{equation} 
which implies that the partition function satisfies 
\begin{align}
-\log Z_N
&= \gamma - \log \expec{\e^{-\alpha X - \beta Y}}  \\
&= \gamma - \log \expec{S_n} - \log\Biggpar{1 + 
\frac{\expec{R_n}}{\expec{S_n}}}\;. 
\end{align}
Commutativity of the diagram~\eqref{comdiag_spaces} yields 
\begin{align}
- \log \expec{S_n}
 &= (\Pi_N \circ \cP)(S_n) \\ 
 &= (\PiNBPHZ \circ \cP)(S_n^0) \\
 &= \sum_{p=2}^{n-1} \sum_{k} \frac{(-\alpha)^p}{p!} b_{pp}^{(k)} 
\PiNBPHZ(\Gamma_{pp}^{(k)})\;.
\end{align}
As pointed out above, only the terms $p=2$ and $p=3$ of this expansion diverge 
in the limit $N\to\infty$, and are compensated exactly by the counterterm 
$\gamma$. 

The remainder $R_n$ can be written as 
\begin{equation}
 R_n = \sum_{q=0}^{\lfloor\nicefrac{n}{2}\rfloor} R_{nq}\;, 
 \qquad 
 R_{nq} = \frac{(-\alpha)^{n-2q}(-\beta)^q}{(n-2q)!q!} X^{n-2q}Y^q
 r_{nq}(X,Y)\;,
\end{equation} 
where the functions $r_{nq}$ admit integral representations similar 
to the remainder in~\eqref{eq:Taylor_remainder}. The Cauchy--Schwarz inequality 
yields 
\begin{align}
 \bigabs{\expec{R_n}} 
 &\leqs \sum_{q=0}^{\lfloor\nicefrac n2\rfloor}
 \frac{\abs{\alpha}^{n-2q}\abs{\beta}^q}{(n-2q)!q!}
 \sqrt{\expec{X^{2(n-2q)}Y^{2q}}}
 \sqrt{\expec{r_{nq}^2}}\\
 &= \Biggpar{\frac\eps4}^n
 \sum_{q=0}^{\lfloor\nicefrac n2\rfloor}
 \frac{\bigpar{2C_N^{(2)}}^q}{(n-2q)!q!}
 \sqrt{\expec{X^{2(n-2q)}Y^{2q}}}
 \sqrt{\expec{r_{nq}^2}}
 \;,
 \label{eq:Rn} 
\end{align}
where we have used the expressions~\eqref{eq:alpha_beta_gamma} for $\alpha$ and 
$\beta$. 
The last factor in this bound is comparable to $\expec{S_n}$ by the same 
argument as in~\eqref{eq:CS_remainder}. It thus remains to bound the 
expectations of polynomial terms. 

Let $\cP_0$ denote the linear operator performing all pairwise matchings, but 
without projecting on connected diagrams. Recall that this amounts to taking 
expectations without taking the logarithm. Then we argue that
\begin{align}
  \bigpar{\PiNBPHZ\circ\cP_0}(X^{2n}) 
 &=  \bigpar{\Pi_N \circ \cP_0 \circ \cM \circ \chi_\eta}(X^{2n}) \\
 &=  \sum_{m=0}^n \frac{(2n)!}{(2n-2m)!m!}
 \Biggpar{-\frac{\beta}{\alpha^2}}^m 
 (\Pi_N \circ \cP_0)\bigpar{X^{2n-2m} Y^m} \\
 &= \sum_{m=0}^n \frac{(2n)!}{(2n-2m)!m!} \bigpar{-8C_N^{(2)}}^m 
 \bigpar{\expec{X^{2n-2m} Y^m}}\;.
\end{align}
The point of this observation is that the quantity $\PiNBPHZ\circ\cP_0(X^{2n})$ 
can be estimated with a procedure detailed in~\cite{Berglund_Bruned_19}, based 
on the exposition in~\cite{Hairer_BPHZ}. Indeed, $\cP_0(X^{2n})$ can be written 
as a sum of Feynman diagrams, obtained by pairwise matching of the $8n$ legs of 
$X^{2n}$. The number of these matchings cannot exceed $(8n-1)!!$ --- in fact, it 
is somewhat smaller, due to the condition of all matchings involving different 
vertices. 

Now a straightforward extension of~\cite[Proposition~6.1]{Berglund_Bruned_19} 
shows that whenever $\Gamma$ has strictly positive degree, one has 
\begin{equation}
 \Bigabs{(\Pi_N\tilde\cA\otimes\id) \Delta(\Gamma)}
 \leqs K^{\abs{\cE(\Gamma)}}
\end{equation} 
where $\abs{\cE(\Gamma)}$ is the number of edges of $\Gamma$, and $K$ is a 
constant depending only on the Green function $G = \lim_{N\to\infty}G_N$. Since 
this number grows at most linearly with $n$, we obtain the bound 
\begin{equation}
 \bigpar{C_N^{(2)}}^m \expec{X^{2n-2m}Y^m} 
 \lesssim (8n-1)!! K^{cn} \frac{(2n-2m)!m!}{(2n)!}
 \lesssim \frac{(8n)!(2n-2m)!m!}{(4n)!(2n)!} \widetilde K^{cn}
\end{equation} 
for constants $c, \widetilde K > 0$. 
Inserting in~\eqref{eq:Rn} and using Stirling's formula yields 
\begin{equation}
 \bigexpec{\bigabs{R_n}} 
 \lesssim \eps^n n! \widetilde K^{cn}
 \sqrt{\expec{r_{nq}^2}}\;,
\end{equation} 
so that indeed Sokal's condition~\eqref{eq:bound_Sokal} is satisfied. 

\begin{remark}
In the last computation, we have argued that the sum over $q$ and the sum over 
$m$ behave similarly, though there may be unexpected cancellations between 
terms. This can be circumvented by a applying the same argument as above to a 
whole family of monomials of the form $(\PiNBPHZ\circ\cP_0)(X^{2n-m}Y^m)$, 
which would allow to estimate the expectations of the monomials 
$X^{2(n-2q)}Y^{2q}$ individually. 
\end{remark}



==> asymptotic.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Cumulant expansion}
\label{ssec:cumulant}

Define the centred moments 
\begin{align}
 \mu_n &:= (-1)^n \biggexpec{\biggpar{\alpha \FGfour + \beta \FGtwo}^n} \\
 &= (-1)^n \sum_{m=0}^n \binom{n}{m} \alpha^m \beta^{n-m} A_{nm}\;, &
 A_{nm} &:= \biggexpec{\FGfour^m \FGtwo^{n-m}}\;.  
\end{align} 
As already alluded to, the coefficients $A_{nm}$ can be computed using the 
properties of Wick calculus, by summing over all contractions, that is, all 
pairings of legs of different diagrams (see Example~\ref{ex:PT} for more 
details). For instance, we have 
\begin{align}
 \mu_2 &= \alpha^2 4! \Pi_N \FGIV + \beta^2 2! \Pi_N \FGII\;, \\
 \mu_3 &= -\alpha^3 \binom{4}{2}^3 2^3 \Pi_N \FGVI 
 - 3\alpha^2\beta (4^2\cdot 2\cdot 3!) \Pi_N \FGIIIplus 
 - 3\alpha\beta^2 4!\, \Pi_N \FGIItwice
 - 8\beta^3 \Pi_N \FGtriangle\;.
\end{align}
We see that each $A_{nm}$ has the form of a combinatorial numerical constant 
times the value of a Feynman diagram, obtained by performing all possible 
contractions. In general, $A_{nm}$ may be a linear combination of Feynman 
diagrams, and these diagrams need not all be connected. For instance, $A_{44}$ 
contains the term
\begin{equation}
\label{eq:non-connected} 
3\cdot (4!)^2 \biggpar{\Pi_N \FGIV}^2\;,
\end{equation} 
where the combinatorial factor $3$ counts the number of pairings of the $4$ 
four-vertex diagrams, and each factor $4!$ counts the number of pairwise 
matchings of the legs within each pair. 

The cumulant expansion reads 
\begin{equation}
\label{eq:cumulant} 
 -\log \expec{\e^{-\alpha X - \beta Y - \gamma}}
 = \gamma - \sum_{n=2}^\infty \frac{\kappa_n}{n!}\;,
\end{equation} 
where the coefficients $\kappa_n$ can be computed recursively 
with the Leonov--Shiraev relation 
\begin{equation}
 \kappa_n = \mu_n - \sum_{m=2}^{n-2} \binom{n-1}{m} \kappa_m \mu_{n-m}\;.
\end{equation} 
It will be useful to write 
\begin{equation}
 \kappa_n = (-1)^n \sum_{m=0}^n \binom{n}{m} \alpha^m \beta^{n-m} B_{nm}\;,
\end{equation} 
where the coefficients $B_{nm}$ are again linear combinations of Feynman 
diagrams. The first few cumulants are 
\begin{align}
 \kappa_2 &= \mu_2\;,\\
 \kappa_3 &= \mu_3\;,\\
 \kappa_4 &= \mu_4 - 3\mu_2^2\;,\\
 \kappa_5 &= \mu_5 - 10\mu_2\mu_3\;.
\end{align}
An important observation is that $\kappa_n - \mu_n$ is always either zero, or a 
sum of products of at least two factors. In terms of Feynman diagrams, this 
means that $\kappa_n - \mu_n$ is a linear combination of non-connected graphs. 

In particular, we see that the term $- 3\mu_2^2$ kills exactly the non-connected 
term~\eqref{eq:non-connected} of $\mu_4$. Therefore, $\kappa_4$ is represented 
by a linear combination of \emph{connected} Feynman diagrams. The fact that this 
generalises to all cumulants is well known in the quantum field theory 
literature, though full proofs seem not easy to find. See 
however~\cite[Sect.~3]{Brouder09}, or~\cite[Sect.~4.2]{Rivasseau_09}.

\begin{proposition} \label{conj:1}
Every $\kappa_n$ is a linear combination of \emph{connected} Feynman diagrams. 
\end{proposition}

The next subsection is dedicated to a proof of this statement.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A combinatorial proof of Proposition~\ref{conj:1}}
\label{ssec:combinatorial_peccati_taqqu}

With~$X$ and~$Y$ as introduced in~\eqref{def:XY}, we set 
\begin{align}
X & \equiv \FGfour \equiv \int_{\T^3} \Wick{\phi(x)^4}\6x =: \int_{\T^3} X(x) 
\6x\;, \quad X(x) := \FGfourlabel{x}\;,\\
Y & \equiv \FGtwo \equiv \int_{\T^3} \Wick{\phi(x)^2}\6x =: \int_{\T^3} Y(x) 
\6x\;, \quad Y(x) := \FGtwolabel{x}\;, 
\end{align} 
and by~$\mu_N$ we always denote the Gaussian Free Field (GFF) at cut-off 
level~$N$, i.e. the centered Gaussian measure on~$L^2(\Lambda)$ with covariance 
kernel~$G_N(x,y) = G_N(x-y)$ given in~\eqref{eq:cov_gff_N}.

We also define
\begin{equation}
\tilde{G}_N(x) := \sum_{k \in \mathcal{K}_N} \frac{1}{\sqrt{\lambda_k + 1}} 
e_k(x)
\end{equation} 
so that~$(\tilde{G}_N * \tilde{G}_N)(x) = G_N(x)$ when~$*$ denotes 
convolution, as can be verified by a straightforward calculation.

Whenever no explicit measure is mentioned, the reference measure is always that 
of spatial white noise on~$L^2(\Lambda)$, i.e., the centred Gaussian measure 
with covariance given by the Dirac kernel~$\delta(x-y)$.
%
Accordingly, we write~$\phi \sim \mu$ as  
\begin{equation}
\phi(x) = I_1\bigpar{\tilde{G}_N(x-\cdot)} 
=: \int_\Lambda \tilde{G}_N(x-z) \xi(\6z)\;,
\label{eq:phi}
\end{equation}
where~$I_1$ is the first Wiener-It\^{o} isometry with respect to spatial white 
noise, see for example the textbook by Nua\-lart~\cite{nualart2006malliavin}.
%
Note that this is consistent with the calculation
\begin{align}
\E^{\mu_N}\biggpar{\phi(x)\phi(y)}
& = 
G_N(x-y) 
=
(\tilde{G}_N * \tilde{G}_N)(x-y)
=
\int_\Lambda 
\tilde{G}_N(z) \tilde{G}_N(z-(x-y)) \6 z \\
& 
=
\int_\Lambda 
\tilde{G}_N(x-z) \tilde{G}_N(y-z) \6 z
=
\E \biggpar{I_1\bigpar{\tilde{G}_N(x-\cdot)} 
I_1\bigpar{\tilde{G}_N(y-\cdot)} }\;,
\end{align}
where we have used that~$G_N$ is even, i.e.~$G_N(x) = G_N(-x)$, and translation 
invariance in the penultimate step.

It is well-known that products of stochastic integrals such as~$\phi$ in 
\eqref{eq:phi} produce correction terms in lower order Wiener-It\^{o} chaoses 
(see e.g.~\cite[Prop.~$1.1.3$]{nualart2006malliavin}) --- but the Wick product 
is the projection onto the highest component, so we have
\begin{equation}
X(x) = \Wick{\phi(x)^4} = I_4(\tilde{G}_N(x-\cdot)^{\otimes 4})\;, \quad
Y(x) = \Wick{\phi(x)^2} = I_2(\tilde{G}_N(x-\cdot)^{\otimes 2})\;.
\end{equation}
Recall that 
\begin{equation}
\kappa(X_1,\ldots,X_n) 
:= \left.\frac{\partial^n}{\partial t_1 \dots \partial t_n} \log 
\E\biggpar{\exp\biggpar{\sum_{\ell=1}^n t_\ell X_\ell}}\right|_{t_1 = \ldots t_n 
= 0}
\end{equation}
denotes the~\emph{cumulant functional}. 
%
With~$\kappa_n(X) = \kappa(X, \ldots, X)$ where~$\kappa$ has $n$ entries, we 
will use the well-known binomial-type formula 
\begin{align}
\kappa_n(\alpha X + \beta Y)
& = 
\sum_{k=0}^n \binom{n}{k} \alpha^k \beta^{n-k} 
\kappa(\underbrace{X,\ldots,X}_{k~\text{times}},\underbrace{Y,\ldots,Y}_{
(n-k)~\text{times}})\;.
\end{align}
Multi-linearity of~$\kappa$ also gives
\begin{equation}
\kappa(\underbrace{X,\ldots,X}_{k~\text{times}},\underbrace{Y,\ldots,Y}_{
(n-k)~\text{times}})
=
\int_{\Lambda^n} 
\kappa\bigpar{X(x_1),\ldots,X(x_k),Y(x_{k+1}),\ldots,Y(x_n)}\; 
\6x_{1:n}
\end{equation}
where~$\6 x_{1:n} := \6 x_1 \ldots \6 x_n$.
%
The following theorem implies the validity of Proposition~\ref{conj:1}.

\begin{theorem} \label{thm:cumu_graphs}
The identity
\begin{equation}
\kappa(\underbrace{X,\ldots,X}_{k~\text{times}},\underbrace{Y,\ldots,Y}_{
(n-k)~\text{times}})
=
\sum_{\Gamma \in \cG} \Pi_N \Gamma
\end{equation}
holds, where~$\cG = \cG(k,n)$ denotes the set of connected 
multigraphs without self-loops that correspond to pairwise matchings.
\end{theorem}

We will not introduce all the terminology in the previous statement abstractly, 
but rather illustrate it in a specific case.
%
As the reader will see, the arguments easily generalise to all combinations 
of~$k$ and~$n$ and thus lead to a \enquote{proof by example.}
%
\begin{remark}
Essentially, the previous theorem is a direct consequence 
of~\cite[Coro.~$7.3.1$]{Peccati_Taqqu_book}, a ge\-ne\-ra\-li\-sa\-tion of 
Wick's theorem followed by a projection onto~\enquote{connected diagrams} to 
account for the cumulant.
%
Since the whole book~\cite{Peccati_Taqqu_book} is written in the language of 
set-partition combinatorics, we hope our example aids the reader in seeing the 
connections clearly.
\end{remark}

\begin{example}[$k=2, n=3$: \enquote{Proof} of Theorem~\ref{thm:cumu_graphs}]
\label{ex:PT} 
We consider
\begin{align}
X(x_1) & = \FGfourlabel{x_1} =   
I_4(\underbrace{\tilde{G}_N(x_1-\cdot)^{\otimes 
4}}_{=: f_1(x_1;\;\cdot)}) \quad \rightarrowtriangle \quad n_1 = 4\;, \\
X(x_2) & = \FGfourlabel{x_2} =  I_4(\underbrace{\tilde{G}_N(x_2-\cdot)^{\otimes 
4}}_{=: f_2(x_2;\;\cdot)}) \quad \rightarrowtriangle \quad n_2 = 4\;, \\
Y(x_3) & = \FGtwolabel{x_3} =  I_2(\underbrace{\tilde{G}_N(x_3-\cdot)^{\otimes 
2}}_{=: f_3(x_3;\;\cdot)}) \quad \rightarrowtriangle \quad n_3 = 2\;.
\end{align}
\begin{enumerate}[label=(\arabic*)]
\item In a first step, we convert the legs of the diagrams~$X(x_i)$, $i=1,2$, 
and~$Y(x_3)$ into nodes and keep the 
label~$x_i$ on the left side of the row. 
%
Accordingly, we have $n= \sum_{i=1}^3 n_i = 10$ nodes in the following diagram: 
%
\begin{center}
\begin{tikzpicture}  
[scale=.8,auto=center,dot/.style={circle,draw=black,fill=black!20}] 
% here, 
% node/.style is the style pre-defined, that will be the default layout of all 
% the nodes. You can also create different forms for different nodes.  

\node (g1) at (-3,6) {$\FGfourlabel{x_1} \quad \rightarrowtriangle \quad$};  
\node (g2) at (-3,4.5) {$\FGfourlabel{x_2} \quad \rightarrowtriangle \quad$};  
\node (g3) at (-3,3) {$\FGtwolabel{x_3} \quad \rightarrowtriangle \quad$};  
\node[dot, label={[label distance=1.5mm] west:$x_1$}] (a1) at (0,6) {};  
\node[dot] (a2) at (2,6)  {}; 
\node[dot] (a3) at (4,6)  {};  
\node[dot] (a4) at (6,6) {};  
\node[dot, label={[label distance=1.5mm] west:$x_2$}] (a5) at (0,4.5)  {};  
\node[dot] (a6) at (2,4.5)  {};  
\node[dot] (a7) at (4,4.5)  {};  
\node[dot] (a8) at (6,4.5)  {};  
\node[dot, label={[label distance=1.5mm]  west:$x_3$}] (a9) at (0,3)  {};  
\node[dot] (a10) at (2,3)  {};  

\end{tikzpicture} 
\end{center}
%
\item We form pairwise matchings of these nodes, signified by 
lines between two nodes, abi\-ding by the following rules:
\begin{enumerate}[label=(\roman*)]
\item One must not match two nodes that are in the same 
row. This would correspond to self-loops in the associated graphs. Peccati and 
Taqqu call these matchings \enquote{non-flat.}
\item The resulting matchings must be such that one cannot 
divide the rows without intersecting one line that symbolises a matching of two 
nodes. 
%
Otherwise, one could partition the rows into two or more 
subsets of rows and form pairwise matchings within each subset. This would 
correspond to disconnected graphs.
\end{enumerate}
The set that contains all of these matchings is 
called~$\mathcal{M}_2([n],\pi^\star)$ by Peccati and Taqqu, see 
point~\ref{it:part_pistar} below for the definition of~$\pi^\star$ in our 
context. 

We denote the specific matching in the following diagram by~$\sigma$: 
%
\begin{center}
\begin{tikzpicture}  
[scale=.8,auto=center,dot/.style={circle,draw=black,fill=black!20}, 
zero/.style={circle,radius=0pt,draw=black,fill=black!100, inner sep=0pt, outer 
sep=0pt, minimum size=.0cm}]] 
% here, node/.style is the style pre-defined, that 
% will be the default layout of all the nodes. You can also create different forms 
% for different nodes.  

\node[dot, label={[label distance=1.5mm] west:$x_1$}] (a1) at (0,6) {};  
\node[dot] (a2) at (2,6)  {}; 
\node[dot] (a3) at (4,6)  {};  
\node[dot] (a4) at (6,6) {};  
\node[dot, label={[label distance=1.5mm] west:$x_2$}] (a5) at (0,4.5)  {};  
\node[dot] (a6) at (2,4.5)  {};  
\node[dot] (a7) at (4,4.5)  {};  
\node[dot] (a8) at (6,4.5)  {};  
\node[dot, label={[label distance=1.5mm]  west:$x_3$}] (a9) at (0,3)  {};  
\node[dot] (a10) at (2,3)  {};  


\draw[red] (a1) -- (a10);
\draw[red] (a2) -- (a5);  
\draw[red] (a3) -- (a7);  
\draw[red] (a4) -- (a8);  
\draw[red] (a6) -- (a9);  

%%%%%%%%%%%%

\node[zero, label={[label distance=1.5mm] \textcolor{red}{$1$}}] (1) at (0,5) 
{};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$2$}}] (2) at (1.8,5) 
{};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$3$}}] (3) at 
(0.8,2.8) {};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$4$}}] (4) at 
(4.3,4.75) {};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$5$}}] (5) at 
(6.3,4.75) {};

\end{tikzpicture} 
\end{center}
%
\item One converts back these matchings into pairings of the 
legs of the variables~$X(x_1)$, $X(x_2)$, and~$Y(x_3)$. For the specific 
matching $\sigma$ above, this leads to the following multigraph (or 
\emph{vacuum Feynman diagram}): 
%
\iffalse
\begin{center}
\begin{minipage}{0.55\textwidth}
\begin{tikzpicture}  
[scale=.7,auto=center,dot/.style={circle,draw=black,fill=black!100, inner 
sep=1.5pt, outer sep=0pt}, 
zero/.style={circle,radius=0pt,draw=black,fill=black!100, inner sep=0pt, outer 
sep=0pt, minimum size=.0cm}] 
% here, node/.style is the style pre-defined, that 
%will be the default layout of all the nodes. You can also create different 
%forms for different nodes.  

\path[use as bounding box] (-2.6,1.1) rectangle (8.1,7.6);


\node[dot, label={[label distance=1.5mm] west:$x_1$}] (a1) at (0,3) {};  
\node[dot, label={[label distance=1.5mm] west:$x_2$}] (a2) at (4,3)  {}; 
\node[dot, label={[label distance=1.5mm] west:$x_3$}] (a3) at (8,3)  {};  
%
\node[zero] (1ol) at (-1,4) {};
\node[zero] (1or) at (1,4) {};
\node[zero] (1ul) at (-1,2) {};
\node[zero] (1ur) at (1,2) {};

%
\draw[thick] (1ol) -- (a1);
\draw[thick] (1or) -- (a1);
\draw[thick] (1ul) -- (a1);
\draw[thick] (1ur) -- (a1);
%
\node[zero] (2ol) at (3,4) {};
\node[zero] (2or) at (5,4) {};
\node[zero] (2ul) at (3,2) {};
\node[zero] (2ur) at (5,2) {};
%
\draw[thick] (2ol) -- (a2);
\draw[thick] (2or) -- (a2);
\draw[thick] (2ul) -- (a2);
\draw[thick] (2ur) -- (a2);
%
\node[zero] (3o) at (8,4) {};
\node[zero] (3u) at (8,2) {};
%
\draw[thick] (3u) -- (a3);
\draw[thick] (3o) -- (a3);

%%%%%%%%%%%%

\draw[red, thick] (1or) to[out=45,in=135] (2ol);
\draw[red, thick] (1ur) to[out=-45,in=-135] (2ul);
\draw[red, thick] (2ur) to[out=-45,in=-90] (3u);
\draw[red, thick] (1ol) to[out=135,in=45] (2or);
\draw[red, thick] (1ul) to[out=225,in=-90] (-2.5,4) to[out=90,in=90] (3o); 

%%%%%%%%%%%%

\node[zero, label={[label distance=1.5mm] \textcolor{red}{$4$}}] (4) at (2,3.5) 
{};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$5$}}] (5) at (2,1.4) 
{};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$2$}}] (2) at (2,5) 
{};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$1$}}] (1) at (2,6.8) 
{};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$3$}}] (3) at (6.5,1) 
{};

\drawbox;

\end{tikzpicture} 
\end{minipage}%
\begin{minipage}{.07\textwidth}%
$\equiv$
\end{minipage}%
\begin{minipage}{.3\textwidth}
\begin{tikzpicture}[scale=2]
\path[use as bounding box] (-0.3, -0.2) rectangle (0.95,0.8);
\draw[semithick] (0,0)--(0.65,0);
\draw[semithick] (0,0) edge [out=60,in=120] (0.65,0);
\draw[semithick] (0,0) edge [out=-60,in=-120] (0.65,0);
\draw[semithick] (0,0) edge [out=80,in=-160] (0.325,0.5);
\draw[semithick] (0.65,0) edge [out=100,in=-20] (0.325,0.5);
\TreeVertex{0}{0};
\TreeVertex{0.65}{0};
\TreeVertex{0.325}{0.5};
\node[] at (-0.2,-0.05) {\footnotesize{$x_1$}};
\node[] at (0.83,-0.05) {\footnotesize{$x_2$}};
\node[] at (0.32,0.66) {\footnotesize{$x_3$}};
%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[] at (0,0.35) {\footnotesize{$\textcolor{gray}{1}$}};
\node[] at (0.325,0.25) {\footnotesize{$\textcolor{gray}{2}$}};
\node[] at (0.65,0.35) {\footnotesize{$\textcolor{gray}{3}$}};
\node[] at (0.325,0.08) {\footnotesize{$\textcolor{gray}{4}$}};
\node[] at (0.325,-0.25) {\footnotesize{$\textcolor{gray}{5}$}};
\drawbox;
\end{tikzpicture}
\end{minipage}
\end{center}
\fi
%
\begin{equation}
\raisebox{-12mm}{
\begin{tikzpicture}  
[scale=.7,auto=center,dot/.style={circle,draw=black,fill=black!100, inner 
sep=1.5pt, outer sep=0pt}, 
zero/.style={circle,radius=0pt,draw=black,fill=black!100, inner sep=0pt, outer 
sep=0pt, minimum size=.0cm}] 
% here, node/.style is the style pre-defined, that 
%will be the default layout of all the nodes. You can also create different 
%forms for different nodes.  

\path[use as bounding box] (-2.6,1.1) rectangle (8.1,7.6);


\node[dot, label={[label distance=1.5mm] west:$x_1$}] (a1) at (0,3) {};  
\node[dot, label={[label distance=1.5mm] west:$x_2$}] (a2) at (4,3)  {}; 
\node[dot, label={[label distance=1.5mm] west:$x_3$}] (a3) at (8,3)  {};  
%
\node[zero] (1ol) at (-1,4) {};
\node[zero] (1or) at (1,4) {};
\node[zero] (1ul) at (-1,2) {};
\node[zero] (1ur) at (1,2) {};

%
\draw[thick] (1ol) -- (a1);
\draw[thick] (1or) -- (a1);
\draw[thick] (1ul) -- (a1);
\draw[thick] (1ur) -- (a1);
%
\node[zero] (2ol) at (3,4) {};
\node[zero] (2or) at (5,4) {};
\node[zero] (2ul) at (3,2) {};
\node[zero] (2ur) at (5,2) {};
%
\draw[thick] (2ol) -- (a2);
\draw[thick] (2or) -- (a2);
\draw[thick] (2ul) -- (a2);
\draw[thick] (2ur) -- (a2);
%
\node[zero] (3o) at (8,4) {};
\node[zero] (3u) at (8,2) {};
%
\draw[thick] (3u) -- (a3);
\draw[thick] (3o) -- (a3);

%%%%%%%%%%%%

\draw[red, thick] (1or) to[out=45,in=135] (2ol);
\draw[red, thick] (1ur) to[out=-45,in=-135] (2ul);
\draw[red, thick] (2ur) to[out=-45,in=-90] (3u);
\draw[red, thick] (1ol) to[out=135,in=45] (2or);
\draw[red, thick] (1ul) to[out=225,in=-90] (-2.5,4) to[out=90,in=90] (3o); 

%%%%%%%%%%%%

\node[zero, label={[label distance=1.5mm] \textcolor{red}{$4$}}] (4) at (2,3.5) 
{};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$5$}}] (5) at (2,1.4) 
{};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$2$}}] (2) at (2,5) 
{};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$1$}}] (1) at (2,6.8) 
{};
\node[zero, label={[label distance=1.5mm] \textcolor{red}{$3$}}] (3) at (6.5,1) 
{};

\drawbox;
\end{tikzpicture} 
}
\qquad\equiv\qquad
\raisebox{-3mm}{
\begin{tikzpicture}[scale=2]
\path[use as bounding box] (-0.3, -0.2) rectangle (0.95,0.8);
\draw[semithick] (0,0)--(0.65,0);
\draw[semithick] (0,0) edge [out=60,in=120] (0.65,0);
\draw[semithick] (0,0) edge [out=-60,in=-120] (0.65,0);
\draw[semithick] (0,0) edge [out=80,in=-160] (0.325,0.5);
\draw[semithick] (0.65,0) edge [out=100,in=-20] (0.325,0.5);
\TreeVertex{0}{0};
\TreeVertex{0.65}{0};
\TreeVertex{0.325}{0.5};
\node[] at (-0.2,-0.05) {\footnotesize{$x_1$}};
\node[] at (0.83,-0.05) {\footnotesize{$x_2$}};
\node[] at (0.32,0.66) {\footnotesize{$x_3$}};
%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[] at (0,0.35) {\footnotesize{$\textcolor{gray}{1}$}};
\node[] at (0.325,0.25) {\footnotesize{$\textcolor{gray}{2}$}};
\node[] at (0.65,0.35) {\footnotesize{$\textcolor{gray}{3}$}};
\node[] at (0.325,0.08) {\footnotesize{$\textcolor{gray}{4}$}};
\node[] at (0.325,-0.25) {\footnotesize{$\textcolor{gray}{5}$}};
\drawbox;
\end{tikzpicture}
}
\end{equation}
%
\item \label{it:part_pistar}There is an analytical expression corresponding to 
this multi-graph respectively the mat\-ching that leads to it. Let us 
illustrate how this can be obtained using the result of Peccati and 
Taqqu~\cite[Coro.~$7.3.1$]{Peccati_Taqqu_book}.

\begin{enumerate}[label=(4.\arabic*)]
\item Note that
\begin{equation}
\biggpar{\bigotimes_{k=1}^3 f_k(x_k,\cdot)}(z_{1:n})
=
f_1(x_1,z_{1:4}) f_2(x_2,z_{5:8}) f_3(x_3,z_{9:10})\;.
\label{eq:fct_tp}
\end{equation}
The partition~$\pi^\star$ in Peccati's and Taqqu's book corresponds exactly to 
the partitioning of the indices of the~$z_i$'s:
\begin{align}
\pi^\star  
& = \bigset{\{1,\ldots,n_1\}, \{n_1+1,\ldots,n_1+n_2\}, 
\{n_1+n_2+1,\ldots,n_1+n_2+n_3\}} \\
& = \bigset{\{1,\ldots,4\}, \{5,\ldots,8\},\{9,10\}}\;.
\end{align}
\item 
The function~$f_{\sigma,\ell} \equiv f_{\sigma,3}$
built from~\eqref{eq:fct_tp} is obtained by simply identifying 
the variables that are matched via~$\sigma$.
%
In precise terms, this means that
\begin{align}
f_{\sigma,3}(z_1,\ldots,z_5)
{}={}& 
\tilde{G}_N(x_1-z_1)\tilde{G}_N(x_1-z_2)
\tilde{G}_N(x_1-z_4)\tilde{G}_N(x_1-z_5) \\
&{}\times \tilde{G}_N(x_2-z_2)\tilde{G}_N(x_2-z_3)
\tilde{G}_N(x_2-z_4)\tilde{G}_N(x_2-z_5) \\
&{}\times \tilde{G}_N(x_3-z_1)\tilde{G}_N(x_3-z_3)\;.
\end{align} 
\item We then find
\begin{equation}
\int_{\Lambda^5} f_{\sigma,3}(z_{1:5}) \6 z_{1:5}
=
G_N(x_2-x_1)^3 G_N(x_3-x_1) G_N(x_3 - x_2)
=
\FGIIIpluslabel{x_1}{x_2}{x_3}
\end{equation}
by repeatedly using the identity $(\tilde{G}_N * \tilde{G}_N)(x) 
= G_N(x)$.
\item Integrating over all the~$x_i$'s (above called the 
\emph{valuation}~$\Pi_N$) we then find
\begin{align}
\int_{\Lambda^3} \int_{\Lambda^5} f_{\sigma,3}(z_{1:5}) 
\6 z_{1:5} \6 x_{1:3}
& =
\int_{\Lambda^3} G_N(x_2-x_1)^3 G_N(x_3-x_1) G_N(x_3 - 
x_2)  \6 x_{1:3} \\
& =
\int_{\Lambda^{\abs{\cV}}} \prod_{e \in \cE} G_N(x_{e_+} 
- x_{e_-})  \6 x
=
\Pi_N \Gamma
\end{align}
for
\begin{equation}
\Gamma
=
\FGIIIplus\;.
\end{equation}
In the literature, the previous drawing sometimes sym\-bo\-li\-ses~$\Gamma \in 
\cG$ and sometimes denotes~$\Pi_N \Gamma \in \R$. 
%
We follow the former convention.
\end{enumerate}
\end{enumerate}
The above procedure clearly generalises to arbitrary values of~$n$ and~$k$ 
and to different matchings that produce~$\Gamma \in \cG = \cG(k,n)$. 
%
Therefore, Theorem~\ref{thm:cumu_graphs} follows by the same route.
\end{example}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{BPHZ renormalisation}
\label{ssec:BPHZ}

We now examine the cumulant expansion~\eqref{eq:cumulant} in more detail.
Each coefficient $A_{nm}$ and $B_{nm}$ is a linear combination of Feynman 
diagrams $\Gamma^{(k)}_{nm}$ having each 
\begin{itemize}
\item $m$ vertices of degree $4$,
\item $n-m$ vertices of degree $2$, 
\item $n+m$ edges.
\end{itemize}
We associate with a multigraph $\Gamma = (\cV, \cE)$ a degree given by 
\begin{equation}
\deg(\Gamma) = 3(\abs{\cV}-1) - \abs{\cE}\;,
\end{equation} 
so that $\deg(\Gamma^{(k)}_{nm}) = 2n - m - 3$ for all $k$. We call a 
diagram $\Gamma$ \emph{divergent} if $\deg\Gamma\leqs0$. 

For small divergent diagrams, one can check that their value diverges 
like $N^{-\deg(\Gamma)}$, possibly with logarithmic corrections. This is 
however not true for many larger diagrams, because of the presence of divergent 
subdiagrams. In fact, there is only one possible divergent subdiagram in our 
situation, namely the \lq\lq bubble\rq\rq\ 
\begin{equation}
\FGIII\;,
\end{equation}
the value of which diverges like $\log N$. 

BPHZ renormalisation, named after Bogoliubov, Parasiuk, Hepp and 
Zimmermann~\cite{Bogoliubow_Parasiuk,Hepp66,Zimmermann69} provides a way of 
dealing with these divergent subdiagrams. It can be formulated in a convenient 
way by using the Connes--Kreimer extraction-contraction coproduct on graphs
\cite{Connes_Kreimer_2000a,Connes_Kreimer_2001}, given by
\begin{equation}
\label{eq:ec_coproduct} 
\Delta(\Gamma) =  \Gamma\otimes\unit + \unit\otimes\Gamma 
+ \sum_{\unit\neq\overline\Gamma\subsetneq\Gamma} 
\overline\Gamma\otimes(\Gamma/\overline\Gamma)\;, 
\end{equation} 
where $\unit$ denotes the empty graph, the sum ranges over all divergent 
subdiagrams, and $\Gamma/\overline\Gamma$ is obtained by contracting all edges 
in $\overline\Gamma$ to one vertex. We further define a (twisted) antipode $\cA$ 
as the linear map satisfying $\cA(\unit) = \unit$, and extended inductively by 
\begin{align}
\cA(\Gamma) 
&= -\cM(\cA\otimes\id)(\Delta\Gamma - \Gamma\otimes\unit) \\
&= -\Gamma - \sum_{\unit\neq\overline\Gamma\subsetneq\Gamma} 
\cA(\overline\Gamma)\cdot(\Gamma/\overline\Gamma)\;, 
\label{eq:antipode} 
\end{align} 
where the product $\cdot$ denotes the disjoint union of graphs, and 
$\cM(\Gamma_1\otimes\Gamma_2) = \Gamma_1\cdot\Gamma_2$. 
For instance, 
\begin{align}
\Delta\Bigpar{\FGIIIplus} &= \FGIIIplus\otimes\unit 
+ \unit\otimes\FGIIIplus + \FGIII \otimes \FGII\;,\\
\cA\Bigpar{\FGIIIplus} &= - \FGIIIplus + \FGIII \cdot \FGII\;.
\label{eq:antipode_FGIIIplus} 
\end{align}
A \emph{character} is by definition a linear form $g:\cG\to\R$, 
$\Gamma\mapsto\pscal{g}{\Gamma}$ which is also multiplicative, in the sense 
that 
\begin{equation}
\pscal{g}{\Gamma_1\cdot\Gamma_2} = 
\pscal{g}{\Gamma_1}\pscal{g}{\Gamma_2}
\qquad \forall\Gamma_1, \Gamma_2\in\cG\;.
\end{equation} 
To such a character, we can associate a renormalisation transformation, given 
by the linear map $M^g: \cG\to\cG$ defined by  
\begin{equation}
M^g(\Gamma) := (g\otimes\id)\Delta\Gamma\;.
\end{equation} 
The \emph{BPHZ character} is given by 
\begin{equation}
\pscal{g^{\text{BPHZ}}}{\Gamma} := 
\begin{cases}
\Pi_N\cA(\Gamma) & \text{if $\deg\Gamma\leqs0$\;,} \\
0 & \text{otherwise\;.}
\end{cases}
\end{equation}
We then define 
\begin{align}
\label{eq:PiNBPHZ} 
\PiNBPHZ(\Gamma) 
&= \Pi_N M^{g^{\text{BPHZ}}} (\Gamma) \\
&= (g^{\text{BPHZ}}\otimes\Pi_N) \Delta\Gamma\;. 
\end{align} 
A compact way of writing this is to introduce the map $\tilde\cA$ defined by 
\begin{equation} \label{eq:tildeA}
\tilde\cA(\Gamma) := \cA(\Gamma) 1_{\deg\Gamma\leqs0}\;,
\end{equation} 
which implies 
\begin{align}
\label{eq:PiNBPHZ} 
\PiNBPHZ(\Gamma) 
&= (\Pi_N\otimes\Pi_N)(\tilde\cA\otimes\id) \Delta\Gamma \\
&= (\Pi_N\tilde\cA\otimes\Pi_N)\Delta\Gamma\;. 
\end{align} 
The following commutative diagram summarises the situation: 
\begin{equation}
\begin{tikzcd}[column sep=large, row sep=large]
\displaystyle \cG
\arrow[r, "\Pi_N"]
\arrow[d, "(\tilde\cA\otimes\id)\Delta"'] 
\arrow[rd, "\PiNBPHZ"]
\arrow[dd, out=180, in=180, distance=50pt, 
" M^{g^{{\text{BPHZ}}}} = (\Pi_N\tilde\cA\otimes\id)\Delta"']
& \R  \\
\displaystyle \cG\otimes\cG
\arrow[r, "\quad\Pi_N\otimes\Pi_N\qquad"] 
\arrow[d, "\Pi_N\otimes\id"'] 
& \R 
\\
\cG
\arrow[ru, "\Pi_N"']
\end{tikzcd}
\end{equation}

The interest of this construction is that one can show that $\PiNBPHZ(\Gamma)$ 
is bounded uniformly in $N$ if $\Gamma$ is non-divergent, and otherwise diverges 
like $N^{-\deg(\Gamma)}$, possibly with logarithmic 
corrections~\cite{Hairer_BPHZ,Berglund_Bruned_19}. 

The aim of the remainder of this section is to give a mostly algebraic proof of 
the following combinatorial result. 

\begin{theorem}
\label{thm:combinatorial} 
For $0 \leqs m \leqs n$, write 
\begin{equation}
B_{nm} = \sum_k b^{(k)}_{nm} \Pi_N\bigpar{\Gamma^{(k)}_{nm}}\;, 
\end{equation} 
where each sum runs over finitely many $k$, the $b^{(k)}_{nm}$ are 
combinatorial coefficients, and each $\Gamma^{(k)}_{nm}$ is a connected Feynman 
diagram with $m$ vertices of degree $4$, $n-m$ vertices of degree $2$, and 
$n+m$ edges. Then 
\begin{equation}
\label{eq:conj2} 
\sum_{n=2}^\infty \frac{\kappa_n}{n!}
= -\sum_{p=2}^\infty \frac{1}{p!} (-\alpha)^p 
\sum_k b^{(k)}_{pp} \PiNBPHZ\bigpar{\Gamma^{(k)}_{pp}}\;,
\end{equation} 
where equality is in the sense of formal power series. 
\end{theorem}

\begin{corollary}
\label{cor:combinatorial}  
All terms in the asymptotic cumulant expansion~\eqref{eq:cumulant} are bounded 
uniformly in the cut-off $N$. 
\end{corollary}
%
\begin{proof}
Since $\deg(\Gamma^{(k)}_{pp}) = p-3$, the only divergent 
$\Gamma^{(k)}_{pp}$ are those with $p\in\set{2,3}$. The choice of $\gamma$ 
in~\eqref{eq:alpha_beta_gamma} precisely compensates these two terms. The 
result follows at once. 
\end{proof}

\subsection{Zimmermann's forest formula}
\label{ssec:Zimmermann} 

A first step in proving Theorem~\ref{thm:combinatorial} is to obtain a simpler 
expression than~\eqref{eq:antipode} for the twisted antipode. This is provided 
by Zimmermann's forest formula~\cite{Zimmermann69,Hairer_BPHZ}, which reads 
\begin{equation}
\cA(\Gamma) = - \sum_{\cF} (-1)^{\abs{\cF}} \cC_\cF\Gamma\;.
\end{equation} 
Here the sum ranges over all forests $\cF$ not containing $\Gamma$, where a 
\emph{forest} is a set of subgraphs of $\Gamma$ which are pairwise either 
included in one another, or vertex-disjoint. The operator $\cC_\cF$ extracts 
all subgraphs in $\cF$ from $\Gamma$ (for a forest, this operation is 
independent of the order of the elements of $\cF$). 

In our simple situation, forests are just unions of disjoint bubbles. The 
forest formula thus takes the following form: if $\Gamma$ contains $g$ bubbles, 
then 
\begin{equation}
\cA(\Gamma) = - \sum_{S\subset\set{1,\dots,g}} 
(-1)^{\abs{S}} \FGIII^{\abs{S}} \cC_S \Gamma\;,
\end{equation} 
where we write $\cC_S$ for the operation consisting in contracting all bubbles 
labelled by an element of $S$ (for an arbitrary fixed labelling of the 
bubbles). 

As a result, using the fact that 
\begin{equation}
\label{eq:bubble}
\Pi_N \Bigpar{\FGIII} = \frac{\beta}{3\eps^2}
= \frac{\beta}{48\alpha^2}\;,
\end{equation} 
we obtain 
\begin{equation}
\PiNBPHZ\bigpar{\Gamma^{(k)}_{pp}}
= - \sum_{S\subset\set{1,\dots,g}} 
\Biggpar{-\frac{\beta}{48\alpha^2}}^{\abs{S}} 
\Pi_N\bigpar{\cC_S \Gamma^{(k)}_{pp}}\;,
\end{equation} 
where $\cC_S \Gamma^{(k)}_{pp}$ is a diagram with $p-\abs{S}$ vertices, 
$\abs{S}$ of which are of degree $2$. 

% Substituting in the right-hand side of~\eqref{eq:conj2}, we obtain 
% \begin{equation}
%  \sum_{p=2}^\infty \sum_k \sum_{q=0}^{g_k} \sum_{S\colon\abs{S}=q}
%  \frac{(-1)^{p+q}}{p!} \frac{b^{(k)}_{pp}}{48^q}
%  \alpha^{p-2q}\beta^q 
%  \Pi_N\bigpar{\cC_S \Gamma^{(k)}_{pp}}\;,
% \end{equation}
% where $g_k$ is the number of bubbles in $\Gamma^{(k)}_{pp}$.
% Using the change of indices $n = p - q$, $m = p - 2q$ in the left-hand side 
% of~\eqref{eq:conj2}, and identifying coefficients of $\alpha^{p-2q}\beta^q$, 
% we 
% find that~\eqref{eq:conj2} is satisfied if 
% \begin{equation}
%  \sum_k \sum_{S\colon\abs{S}=q} b^{(k)}_{pp}
%  \Pi_N\bigpar{\cC_S \Gamma^{(k)}_{pp}}
%  = \frac{p!48^q}{q!(p-2q)!}
%  \sum_{\ell} b^{(\ell)}_{p-q, p-2q} 
%  \Pi_N\bigpar{\Gamma^{(\ell)}_{p-q, p-2q}}
% \end{equation} 
% holds for each $p \geqs 2$ and each $q\in\set{0,\dots,g_k}$. If the diagrams 
% are 
% consistently numbered, this condition reduces 
% to the simpler condition 
% \begin{equation}
%  b^{(k)}_{pp} = \frac{p!(g-q)!}{g!(p-2q)!} 48^q b^{(k)}_{p-q, p-2q}\;.
% \end{equation} 
% Note that this condition is automatically satisfied for $q=0$. It seems 
% possible to prove it in the general case by a combinatorial argument, based 
% on 
% inserting/extracting bubbles. Again, there may be a more elegant proof based 
% on 
% algebraic properties. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A Hopf-algebra-flavoured proof}
\label{ssec:Hopf}

As we have already alluded to in the last sections, it is well-known that the 
triple~$(\cG,\cdot,\Delta)$ can canonically be turned into a Hopf algebra, 
itself isomorphic to the \emph{Connes--Kreimer Hopf 
algebra}~\cite{ConnesKreimer98} of rooted trees.
%
Therefore, it is natural to expect that a particularly elegant proof of 
Theorem~\ref{thm:combinatorial} may be achieved if one were to interpret $X = 
\FGfour$ and~$Y = \FGtwo$ as \emph{monomials} in a polynomial Hopf algebra.
%
Indeed, such a construction has been performed by Ebrahimi-Fard et 
al.~\cite{EFPTZ18}: In this section, we describe how to adapt it for our 
purposes.\footnote{Note that~$X$ and~$Y$ do satisfy the assumptions in that 
article: They have moments of all orders because probabilistic~$L^p$-norms 
coincide in all homogeneous Wiener-It\^{o} 
chaoses~\cite[Thm.~$3.50$]{Janson_book_08}.}

We let~$\X := (X,Y)$ and for each~$\bn =(n_1,n_2) \in \N^2$ then 
define 
\begin{equation}
\X^{\bn} := X^{n_1}Y^{n_2}\;, \quad 
\X^{(0,0)} := \bs{1}\;, \quad
H := \operatorname{span}\bigset{\X^{\bn}: \ \bn \in \N^2}\;.
\end{equation}

\begin{remark}
In~\cite{EFPTZ18}, the authors allow for~$\X = (X_a: \ a \in 
I)$ where~$I$ is some (possibly infinite) index set and then consider the set
\begin{equation}
M(I) = \bigset{B: I \to \N: \ B(a) \neq 0 \ \text{for 
finitely many} \ a \in \cA}\;.
\end{equation}   
In our setting~$\abs{I} = 2$, so we can identify~$M(I) \simeq \N^2$, 
i.e. we just consider~$B = \bn \in \N^2$.
%
In particular, we still consider polynomials~$\X^{\bn}$ 
as above and, contrary to~\cite{EFPTZ18}, do not base our analysis on the 
(isomorphic) vector space freely generated from~$M(I)$.

We repeat some of the constructions in~\cite{EFPTZ18}, albeit in a way slightly 
adapted to our setting. For~$\bn,\bm, \bk \in \N_0^2$, we define
\begin{align} 
\cM(\X^{\bn} \otimes \X^{\bm})
& := \X^{\bn} \cdot \X^{\bm} 
:= \X^{\bn \cdot \bm}, \quad \bk \cdot \bm 
:= (k_1 + m_1, k_2 + m_2),
  \\
\hat{\Delta} \X^{\bn}  & :=
\sum_{\substack{\bk,\bm \in \N_0^2 \\ \bk \cdot 
\bm = \bn}} \binom{\bn}{\bm,\bk} \X^{\bk} \otimes \X^{\bm}, 
\quad \binom{\bn}{\bm,\bk} := \prod_{i=1}^2 \frac{n_i!}{m_i! k_i!}\;,
\end{align}
with a slight abuse of notation for the product~$\cdot$\thinspace. 
%
It is proved in~\cite{EFPTZ18} that~$\Delta$ defines a coproduct 
on~$H$. 
\end{remark}
%
In the previous sections, we have seen that the (twisted) antipode~$\cA$~(resp.~$\tilde{\cA}$) plays a crucial role in the renormalisation of multigraphs~$\Gamma \in \cG$.
%
In this section, we want to define a corresponding map~$\hat{\cA}_\eta$ acting on~$H$, as well as a map~$\cP$ that sends~$H$ to~$\cG$, such that the following two diagrams between spaces respectively objects commute:


\begin{equation} \label{comdiag_spaces}
\begin{tikzcd}[column sep=large, row sep=large]
H 
\arrow[r, "\cP"] 
\arrow[d, "\chi_\eta = 
(\hat\cA_\eta\otimes\id)\hat\Delta"']
& \displaystyle \cG
\arrow[r, "\Pi_N"]
\arrow[d, "(\tilde\cA\otimes\id)\Delta"'] 
\arrow[rd, "\PiNBPHZ"]
& \R  \\
H\otimes H
\arrow[d, "\cM"'] 
& \displaystyle \cG\otimes\cG
\arrow[r, "\quad\Pi_N\otimes\Pi_N\qquad"] 
%\arrow[d, "\cM_{\text{forest}}"'] 
\arrow[d, "\Pi_N \otimes \id"'] 
& \R 
\\
H
\arrow[r, "\cP"] 
& \cG
\arrow[ru, "\Pi_N"']
\end{tikzcd}
\end{equation}


\begin{equation}  \label{comdiag_objects}
\begin{tikzcd}[cramped,column sep=large, row sep=large]
\e^{-\alpha X} 
\arrow[r, "\cP", mapsto] 
\arrow[d, "\chi_\eta = 
(\hat\cA_\eta\otimes\id)\hat\Delta"', 
mapsto]
& \displaystyle \sum_{n,k} \tfrac{(-\alpha)^n}{n!} b_{nn}^{(k)} 
\Gamma_{nn}^{(k)} 
\arrow[r, "\Pi_N", mapsto]
\arrow[d, "(\tilde\cA\otimes\id)\Delta"', mapsto] 
\arrow[rd, "\PiNBPHZ", mapsto]
& \displaystyle \sum_{n} \tfrac{(-\alpha)^n}{n!} B_{nn}
%b_{nn}^{(k)} \Pi_N(\Gamma_{nn}^{(k)})  
\\
%(\dots) 
\displaystyle
\sum_{n,m} \tfrac{(-\alpha)^n(-\eta)^m}{(n-2m)!m!} Y^m\otimes X^{n-2m}
\arrow[d, "\cM"', mapsto] 
& \displaystyle \sum_{n,k,S} 
\tfrac{(-\alpha)^n}{n!} b_{nn}^{(k)}
\tilde\cA\bigpar{\raisebox{2mm}{\scalebox{0.7}{\FGIII}}^{\abs{S}}} 
\otimes \cC_S \Gamma_{nn}^{(k)}
\arrow[r, "\Pi_N\otimes\Pi_N", mapsto] 
%\arrow[d, "\cM_{\text{forest}}"', mapsto] 
\arrow[d, "\Pi_N \otimes \id"', mapsto] 
& \displaystyle \sum_{n} \tfrac{(-\alpha)^{n-m}(-\beta)^m}{(n-m)!m!} B_{nm} 
%b_{nn}^{(k)}\PiNBPHZ(\Gamma_{nn}^{(k)})  
\\
\e^{-\alpha X - \beta Y}
\arrow[r, "\cP", mapsto] 
& \displaystyle \sum_{n,m,k} 
\tfrac{(-\alpha)^{n-m}(-\beta)^m}{m!(n-m)!} 
b_{nm}^{(k)} 
\Gamma_{nm}^{(k)} 
\arrow[ru, "\Pi_N"', mapsto]
\end{tikzcd}
\end{equation}

The following definition introduces the desired maps~$\hat{\cA}_\eta$ and~$\cP$.
%
Recall that
\begin{equation} \label{eq:double_factorial}
(2\ell-1)!! 
:= \prod_{i=1}^{\ell} (2i-1)
= \frac{(2\ell)!}{2^\ell \ell!}\;.
\end{equation} 

\begin{definition} \label{def:antipode_2}
We define the linear map~$\hat{\cA}_\eta: H \to H$ by 
%\begin{equation}
%\label{eq:antipode2}
%\hat{\cA}_\eta \X^{\bn} := 
%\begin{cases}
%\bs{1} & \quad \text{if} \quad n_1 = n_2 = 0 \quad 
%(\text{i.e. if} \quad \X^{\bn} = \bs{1})\;, \\
%0 & \quad \text{if} \quad n_1 > 0, \ n_2 \geqs 0 \quad 
%(\text{i.e. if} \quad \X^{\bn} = X^{n_1} Y^{n_2})\;,\\
%(-\eta \X)^{\bn} = (-\eta Y)^{n_2} & \quad 
%\text{if} \quad n_1 = 0, \ n_2 > 0  \quad (\text{i.e. 
%if} \quad \X^{\bn} 
%= Y^{n_2})\;.\\
%\end{cases}
%\end{equation}
\begin{equation}
\label{eq:antipode2}
\hat{\cA}_\eta \X^{\bn} := 
\begin{cases}
(2\ell-1)!! (-2 \eta Y)^{\ell} & \quad 
\text{if} \quad n_1 = 2\ell, \ n_2 = 0\;,\\
0 & \quad \text{otherwise}, \\
\end{cases}
\end{equation}
Note that the condition on the first line is satisfied precisely if \;$\X^{\bn} 
= X^{2\ell} \ \text{for some} \ \ell \in \N_0$ and, in particular, implies 
that~$\hat{\cA}_\eta \mathbf{1} = \mathbf{1}$.  
%
We also decree that~$\hat{\cA}_\eta$ is linear w.r.t. infinite sums and define
%
\begin{equation}
\chi_\eta: H \to H \otimes H\;, \quad 
\chi_\eta(\X^{\bn}) := (\hat{\cA}_\eta \otimes 
\id) \hat{\Delta} \X^{\bn} \;,
\end{equation}
%
as well as the operation~$\cP: H \to \cG$ by
\begin{equation}
\cP \X^{\bn} := \sum_{\Gamma \in \cG(n_1,n_1+n_2)} \Gamma\;,
\end{equation}
for\; $\cG(n_1,n_1+n_2)$ as given in Theorem~\ref{thm:cumu_graphs}. 
Note that this corresponds exactly to~$\X^{\bn} = X^{n_1}Y^{n_2}$. In other 
words,~$\cP$ coincides with~$\kappa$ up to taking the valuation~$\Pi_N$.
\end{definition}


\begin{remark}
The previous definition might seem somewhat \enquote{ad-hoc}, so let us 
explain the motivation behind it. 
%
Essentially, we want to mirror the down-facing arrows in the middle 
of~\eqref{comdiag_spaces} and~\eqref{comdiag_objects}, respectively.
%
We neglect combinatorial factors which are accounted for by the 
binomial coefficient. 
\begin{enumerate}[label=(\arabic*)]
\item 
We know that the extraction-contraction co-product~$\Delta$ 
given in \eqref{eq:ec_coproduct} extracts divergent subgraphs of some 
\emph{connected} graph~$\Gamma$. 

The only divergent diagrams in our setting are~$\FGIV$, 
$\FGVI$, and the bubble~$\FGIII$ --- but all the vertices of the first two 
graphs have valence~$4$, so they cannot be subgraphs of~$\Gamma$  because it is 
connected, see also Section~\ref{ssec:Zimmermann}. 

\item The bubble, however, is produced by pairing three of the 
legs of~$X = \FGfour$ with three legs of another instance of~$X$; extracting a 
bubble then locally produces~$\FGIII \cdot \FGtwo$, i.e.~$\eta Y$ for~$\eta 
\simeq \nicefrac{\beta}{\alpha^2}$.
%
Because~\enquote{two instances of~$X$ produce~$Y$}, the latter 
should count double for the argument to be correct; that is the reason for the 
action of~$\hat{\cA}_\eta$ on even powers of~$X$.

\item Encoding the factor~$\eta$ in~$\hat{\cA}_\eta$ (and not~$\hat{\Delta}$) 
seemed more convenient in computations and resembles the action of~$\cA$ 
in~\eqref{eq:antipode_FGIIIplus} more closely.

\item The factor $(2\ell-1)!!$ counts all possible ways to pair the $2\ell$ 
four-vertex diagrams.

\item The map~$\hat{\cA}_\eta$ should act trivially on non-divergent diagrams, 
so it sends all monomials that are not even powers of~$X$ to~$0$.  
\qedhere
\end{enumerate}
\end{remark}


The following proposition proves that the two leftmost down-facing arrows in 
the diagrams \eqref{comdiag_spaces} and~\eqref{comdiag_objects} correspond to 
well-defined operations:

\begin{proposition}
\label{prop:exponential} 
The identity~$(\cM \circ \chi_\eta) \e^{-{\alpha X}} = \e^{-\alpha X - 
\beta Y}$ holds.
\end{proposition}

\begin{proof}
Observe that~$X^n = \X^{\bn}$ for~$\bn = (n_1,n_2) = (n,0)$. By 
definition, we thus have
\begin{equation}
(\cM \circ \chi_\eta)X^n = \sum_{\substack{\bm,\bk \in \N^2 \\ \bm \cdot \bk = 
\bn}} \binom{\bn}{\bm,\bk} \hat{\cA}_\eta (\X^{\bm}) 
\X^{\bk}\;,
\label{eq:cMchi_Xn}
\end{equation}
and since~$n_2 = 0$, the condition~$\bm \cdot \bk = \bn$ implies that~$m_2 + k_2 
= 0$. As~$m_2, k_2 \in \N_0$, we then find~$m_2 = k_2 = 0$ and the preceding 
formula simplifies to
\begin{equation}
(\cM \circ \chi_\eta)X^n 
= \sum_{\substack{m,k \in \N \\ m + k = n}} \frac{n!}{m! k!} \hat{\cA}_\eta 
(X^{m}) 
X^{k}\;
= \sum_{m=0}^n \frac{n!}{m! (n-m)!} \hat{\cA}_\eta (X^{m}) 
X^{n-m}.
\label{eq:cMchi_Xn_2}
\end{equation}
Accounting for the definition of the antipode in~\eqref{eq:antipode2}, we arrive 
at the identity
\begin{align}
(\cM \circ \chi_\eta)X^n 
& = \sum_{\ell=0}^{\lfloor \nicefrac{n}{2} \rfloor} \frac{n!}{(2\ell)! 
(n-2\ell)!} \hat{\cA}_\eta (X^{2\ell}) 
X^{n-2\ell} \\
& = \sum_{\ell=0}^{\lfloor \nicefrac{n}{2} \rfloor} \frac{n!}{(2\ell)! 
(n-2\ell)!} (2\ell-1)!! (-2\eta Y)^{\ell}
X^{n-2\ell} \label{eq:cMchi_Xn_3}\\
& = \sum_{\ell=0}^{\lfloor \nicefrac{n}{2} \rfloor} \frac{n!}{\ell! (n-2\ell)!} 
(-\eta Y)^{\ell}
X^{n-2\ell}.
\end{align}
Next, we expand the exponential function
\begin{equation}
\e^{-\alpha X} = \sum_{n=0}^{\infty} \frac{(-1)^n}{n!} \alpha^n 
X^n\;
\end{equation}
so that the previous computation and~$\eta = 
\nicefrac{\beta}{\alpha^2}$ implies that 
\begin{equation}
(\cM \circ \chi_\eta) \e^{-{\alpha X}} 
=
\sum_{n=0}^{\infty} \frac{(-1)^n}{n!} 
\sum_{\ell = 0}^{\lfloor \nicefrac{n}{2} \rfloor} \frac{n!}{(n-2\ell)! 
\ell!} (- \beta Y)^\ell (\alpha X)^{n-2\ell}\;.
\end{equation}
We now set~$p := n-\ell$ and~$q := n-2\ell$ so that 
\begin{equation}
\ell = p-q\;, \quad n = 2p - q\;, \quad (-1)^n  = (-1)^{n-2\ell} (-1)^{2\ell} 
= (-1)^q \quad \text{for} \quad \ell = 0,\ldots,\lfloor \nicefrac{n}{2} 
\rfloor\;, 
\end{equation}
and then reorganise the series accordingly to get
\begin{align}
(\cM \circ \chi_\eta) \e^{-{\alpha X}} 
& =
\sum_{p=0}^{\infty} 
\sum_{q = 0}^{p} \frac{1}{q! (p-q)!} (- \beta Y)^{p-q} (-\alpha 
X)^q \\
& = 
\sum_{p=0}^{\infty} \frac{1}{p!}
\sum_{q = 0}^{p} \binom{p}{q} (- \beta Y)^{p-q} (-\alpha X)^q 
= \e^{-\alpha X + \beta Y}\;.
\end{align}
The proof is complete.
\end{proof}

\begin{remark}
For~$n \in \{2,3\}$, we have
\begin{equation}
(\cM \circ \chi_\eta)X^2 
= X^2 - 2 \eta Y, \quad
(\cM \circ \chi_\eta)X^3  
= X^3 - 6 \eta YX.
\end{equation}
From these examples, it is interesting to note that, upon identifying
\begin{equation}
X \; \longleftrightarrow \; Z \sim \cN(0,1), \quad E[X^2] \; \longleftrightarrow 
\; 2 \eta Y,
\end{equation}
the map~$\cM \circ \chi_\eta$ behaves like a Wick product. 
%
We leave further investigations of this observation for future work.
\end{remark}

It remains to check that the diagrams are indeed commutative. This is the 
content of the next section.

\subsection{Combinatoric proof of the diagram's commutativity}
\label{ssec:combinatorics}

\iffalse
\begin{equation}  \label{comdiag_Xn}
\begin{tikzcd}[column sep=large, row sep=large]
X^n 
\arrow[r, "\cP", mapsto] 
\arrow[d, "\chi_\eta = 
(\hat\cA_\eta\otimes\id)\hat\Delta"', 
mapsto]
& \displaystyle \sum_{k}  b_{nn}^{(k)} 
\Gamma_{nn}^{(k)} 
% \arrow[r, "\Pi_N", mapsto]
\arrow[d, "(\tilde\cA\otimes\id)\Delta"', mapsto] 
% \arrow[rd, "\PiNBPHZ"', mapsto]
% & \displaystyle \sum_{k} b_{nn}^{(k)} 
% \Pi_N(\Gamma_{nn}^{(k)})  
\\
%(\dots) 
\displaystyle
\sum_{n,m} \tfrac{n!(-\eta)^m}{(n-2m)!m!} Y^m\otimes X^{n-2m}
\arrow[d, "\cM"', mapsto] 
& \displaystyle \sum_{k,S} b_{nn}^{(k)} 
\tilde\cA\Bigpar{\raisebox{2mm}{\FGIII}^{\abs{S}}} \otimes \cC_S 
\Gamma_{nn}^{(k)}
% \arrow[r, "\Pi_N\otimes\Pi_N"', mapsto] 
\arrow[d, "\cM_{\text{forest}}"', mapsto] 
% \arrow[d, "\Pi_N \otimes \id"', mapsto] 
% & \displaystyle \sum_{k} b_{nn}^{(k)} 
% \PiNBPHZ(\Gamma_{nn}^{(k)})  
\\
\displaystyle
\sum_{n,m} \tfrac{n!(-\eta)^m}{(n-2m)!m!} Y^m X^{n-2m}
\arrow[r, "\cP", mapsto] 
& \displaystyle \sum_{k,S} b_{nn}^{(k)} \biggpar{\frac{-\eta}{48}}^{\abs{S}}
\cC_S \Gamma_{nm}^{(k)} 
% \arrow[ru, "\Pi_N"', mapsto]
\end{tikzcd}
\end{equation}
\fi

% [This is a first version of the combinatorical approach to the fact that the 
% above diagram commutes. It may be possible to make the arguments more elegant 
% by using a more algebraic approach.]

To complete the proof of Theorem~\ref{thm:combinatorial}, we need to 
show that the identity
\begin{align}
\label{eq:commutative} 
 \cP \circ \cM \circ \chi_\eta
 &= (\Pi_N\otimes\id)\circ(\tilde\cA\otimes\id)\Delta\circ\cP \\
 &= (\Pi_N\tilde\cA \otimes \id)\Delta \circ \cP
\end{align} 
holds on the space spanned by all monomials $X^n$. This is equivalent to 
showing that the following diagram commutes:
%
\begin{equation}  \label{comdiag_Xn_small}
\begin{tikzcd}[column sep=large, row sep=large]
X^n 
\arrow[r, "\cP", mapsto] 
\arrow[d, "\cM \circ\chi_\eta"', 
mapsto]
& \displaystyle \sum_{k}  b_{nn}^{(k)} 
\Gamma_{nn}^{(k)} 
\arrow[d, "(\Pi_N\otimes\id)(\tilde\cA\otimes\id)\Delta", mapsto] 
\\
\displaystyle
\sum_{n,m} \tfrac{n!(-\eta)^m}{(n-2m)!m!} Y^m X^{n-2m}
\arrow[r, "\cP", mapsto] 
& \displaystyle \sum_{k,S} b_{nn}^{(k)} \Biggpar{\frac{-\eta}{48}}^{\abs{S}}
\cC_S \Gamma_{nm}^{(k)} 
\end{tikzcd}
\end{equation}
%
We have already obtained in the proof of Proposition~\ref{prop:exponential} the 
expression 
\begin{equation}
 (\cM \circ \chi_\eta)(X^n)
 = \sum_{m=0}^{\lfloor n/2 \rfloor} 
 \frac{n!}{(n-2m)!m!}(-\eta)^m Y^m X^{n-2m}\;.
\end{equation} 
On the other hand, recalling that $\eta = \nicefrac{\beta}{\alpha^2}$, we get 
\begin{equation}
 (\Pi_N\tilde\cA \otimes \id)\Delta\Gamma
 = -\sum_{m=0}^{\lfloor n/2 \rfloor} 
 \Biggpar{\frac{\eta}{48}}^m 
 \sum_{S\colon \abs{S} = m} \cC_S\Gamma\;,
\end{equation} 
where the second sum runs over all sets of $m$ bubbles (if $\Gamma$ has fewer 
than $m$ bubbles, the last sum is zero by definition). Comparing the last two 
expressions, we see that~\eqref{eq:commutative} holds if
\begin{equation}
\label{eq:combi_nm} 
 \cP(Y^m X^{n-2m}) 
 = \frac{(n-2m)!m!}{48^m n!}
 \sum_{S\colon \abs{S} = m} \cC_S(\cP X^n) 
\end{equation} 
for any $n\geqs1$. Recall that both sides of this relation involve in general a 
sum over several Feynman diagrams. There is, however, a natural identification 
between these diagrams, so that we may lighten the notation by pretending that 
there is only one diagram in each sum. 

We now observe that $\cP(Y^m X^{n-2m})$ is a (sum of) diagram(s) having $m$ 
vertices of degree $2$, $n-m$ vertices of degree $4$, and $2n-m$ edges. To 
produce the corresponding term on the right-hand side, we argue that instead of 
extracting bubbles on the right-hand side, we can also insert bubbles on the 
left-hand side. This amounts to inserting $2m$ four-vertex diagrams at the 
vertices of degree $2$ of $\cP(Y^m X^{n-2m})$. To do that, there are 
\begin{itemize}
 \item $\binom{n}{2m}$ ways of selecting the $2m$ four-vertex diagrams; 
 \item $(2m-1)!!$ ways to pair the $2m$ four-vertex diagrams;
 \item $4^2\cdot3! = 96$ ways of matching six pairs of legs of each set of two 
four-vertex diagrams, amounting to $96^m$ matchings;
 \item and finally, $m!$ ways of inserting the resulting bubbles at the $m$ 
vertices of index $2$.
\end{itemize}
%Recalling~\eqref{eq:double_factorial} and 
%\begin{equation}
% (2m-1)!! = \frac{(2m)!}{2^m m!}\;,
%\end{equation} 
Multiplying all the above combinatorial factors, by~\eqref{eq:double_factorial} 
we arrive at 
\begin{equation}
 \frac{48^m n!}{m!(n-2m)!}
\end{equation} 
ways of inserting the four-vertex diagrams. This is indeed compatible with the 
desired relation~\eqref{eq:combi_nm}. The proof of 
Theorem~\ref{thm:combinatorial} is complete. 


We close this section with an example that deals with mixed monomials.
\begin{example}
As we have seen, it suffices for the purposes of this article that the diagram 
in~\eqref{comdiag_Xn_small} commutes for the base monomial~$X^n$.
%
However, the following example gives us hope that the commutativity might still 
be true for monomials containing non-trivial powers of~$Y$.

Let~$\X^{\bn} = X^2 Y$, i.e.~$\bn = (n_1,n_2) = (2,1)$.
%
We find
\begin{align}
\hat{\Delta} (X^2 Y) 
& = X^2 Y \otimes \mathbf{1} + \mathbf{1} \otimes X^2 Y + X^2 \otimes Y + Y 
\otimes X^2 + 2  XY \otimes X + 2 X \otimes XY\;, \\
\chi_\eta (X^2 Y) 
& =  \mathbf{1} \otimes X^2 Y + \hat{\cA}_\eta(X^2) \otimes Y\;,
\end{align}
and then
\begin{equation}
\label{eq:computation_mixed_monomial}
(\cM \circ \chi_\eta) (X^2 Y)
=
X^2 Y - 2 \eta Y^2\;.
\end{equation}
Next, note that
\begin{equation}
\label{eq:PXXY} 
\cP(X^2 Y) = 4^2\cdot 2!\cdot 3! \,\FGIIIplus\;, 
\qquad \cP(Y^2) = 2! \,\FGII\;,
\end{equation}
where the combinatorial factor in the first expression counts the $4^2$ ways of 
choosing one leg in each four-vertex diagram, the $2!$ ways of matching these 
with the legs of the two-vertex diagram, and the $3!$ pairwise matchings of the 
remaining legs. 
From~the equalities in~\eqref{eq:antipode_FGIIIplus}, \eqref{eq:tildeA}, as well 
as \eqref{eq:bubble}, we obtain 
\begin{equation}
(\Pi_N\otimes\id)(\tilde\cA\otimes\id)\Delta \FGIIIplus
=
\FGIIIplus - \Pi_N \FGIII \cdot \FGII
=
\FGIIIplus - \frac{\eta}{48} \FGII\;.
\end{equation}
Applying the expressions~\eqref{eq:PXXY} of $\cP$ to $X^2Y$ and $X^2Y-2\eta 
Y^2$, we see that the commutativity relation~\eqref{eq:commutative} is indeed 
satisfied. We expect that the same conclusion holds for other mixed monomials, 
modulo a suitable encoding of the combinatorics in the definition of the 
map~$\hat{\cA}_\eta$ from Definition~\ref{def:antipode_2}.
% Modulo application of~$\cP$, this expression is very similar to the one 
% in~\eqref{eq:computation_mixed_monomial} --- aside from a combinatorial 
% prefactor in the second summand.
% %
% We expect that this deficiency can be remedied by suitably encoding the 
% combinatorics detailed above in the definition of the map~$\hat{\cA}_\eta$ from 
% Definition~\ref{def:antipode_2}.
\end{example}

